Revisi\'on de M\'etodos de Planificaci\'on de Camino de Cobertura para Entornos Agr\'icolas

The use of an efficient coverage planning method is key for autonomous navigation in agricultural environments, where a robot must cover large areas of crops. This paper generally reviews the current state of the art of coverage path planning methods. Two widely used techniques applicable to agricultural environments are described in detail. The first consists of breaking down a complex field with obstacles into simpler subregions known as cells, to subsequently generate a coverage pattern in each of them. The second analyzes spaces composed of parallel strips through which the robot must circulate, in order to find the optimal order of visiting strips that minimizes the total distance traveled. Additionally, the combination of both techniques is discussed in order to obtain a more efficient global coverage plan. This analysis was conceived to be implemented with the soybean crop weeding robot developed at CIFASIS (CONICET-UNR).

==> src/acknowledgment.tex <==
Este trabajo se encuentra en el marco del proyecto \emph{Desarrollo de un Robot Desmalezador} de la Unidad Ejecutora CIFASIS, Centro Internacional Franco Argentino de Ciencias de la Información y de Sistemas (CONICET-UNR).
